Product Title Refinement via Multi-Modal Generative Adversarial Learning

Nowadays, an increasing number of customers are in favor of using E-commerce Apps to browse and purchase products. Since merchants are usually inclined to employ redundant and over-informative product titles to attract customers' attention, it is of great importance to concisely display short product titles on limited screen of cell phones. Previous researchers mainly consider textual information of long product titles and lack of human-like view during training and evaluation procedure. In this paper, we propose a Multi-Modal Generative Adversarial Network (MM-GAN) for short product title generation, which innovatively incorporates image information, attribute tags from the product and the textual information from original long titles. MM-GAN treats short titles generation as a reinforcement learning process, where the generated titles are evaluated by the discriminator in a human-like view.

==> related_work.tex <==
\section{Related Work}

Our work is related to text summarization tasks and generative adversarial networks (GANs). 
\subsection{Text Summarization}
In terms of text summarization, it mainly includes two categories of methods: extractive methods  and abstractive methods. Extractive methods produce  a text summary by extracting and concatenating several words from original sentence. Whereas abstractive methods generate a text summary based the original sentence, which usually generate more readable and coherent summaries.  Traditional extractive methods such as  graphic model \cite{mihalcea2005language} and optimization-based model \cite{woodsend2010automatic} usually rely on human-engineered features. Recent RNN based methods \cite{nallapati2017summarunner,nallapati2017summarunner,chopra2016abstractive} have become popular in text summarization tasks. Among them,  \cite{nallapati2017summarunner} treats summary extraction as a sequence classification problem, where each word is visited sequentially and a binary decision is made to decide whether to choose the visited word into the summary, \cite{cheng2016neural} designs an attention-based RNN model to attend the whole document when extracting a word to the summary. \cite{chopra2016abstractive} is an abstractive method which designs a  convolutional attention-based encoder and RNN decoder to generate summaries. \cite{see2017get} proposes a pointer network to make a balance between extractive and abstractive  and shows promising performance. \cite{wang2018multi,gong2018automatic} design attention-based neural networks for short product titles generation in E-commerce. \cite{gong2018automatic} considers rich semantic features of long product titles. \cite{wang2018multi} designs a multi-task model which uses user searching log data as additional task to help better extractive key words from original long titles. However, they mainly consider information from textual long product titles, which sometimes are not enough to select important words and filter out over-informative and irrelevant words from long product titles. In additional, above methods mainly using MLE objective and predict next word based on previous words. As a consequence, these models usually suffer from exposure bias and lack of human-like view.

\subsection{Generative Adversarial Networks (GANs)}
GAN is first proposed in \cite{goodfellow2014generative}, which is designed for generating real-valued, continuous data, and has gained great success in computer vision tasks \cite{isola2017image,dai2017towards,ledig2017photo}.  However,  applying GANs to discrete space and discrete sentences like texts has encountered many difficulties, because the discrete elements break the differentiability of GANs and prohibit gradients from the discriminator flowing to generator. Due to this reason, GAN has not achiEved comparabke success in NLP. Recently, researchers usually reformulate the problem to continuous domain or consider reinforcement learning problems. 

SeqGan \cite{yu2017seqgan} takes sequence generation procedure as a sequential decision making process. It applies a policy gradient method to train the generator and discriminator, and shows improvements on multiple generation task such as poem generation and music generation. MaskGan \cite{fedus2018maskgan} designs a actor-critic reinforcement learning based GAN to improve qualities of text generation through filling in missing texts conditioned on the surrounding context. There are also some other RL based GANs for text generation such as LeakGan \cite{guo2017long}, RankGan \cite{lin2017adversarial}, SentiGan \cite{wang2018sentigan}, etc. All above methods are designed for unsupervised text generation tasks. 

\cite{li2017adversarial} designs an adversarial learning method for neural dialogue generation. They train a seq2seq model to produce responses and use a discriminator to distinguish whether the responses are human-generated and machine-generated, and showing promising results. They also propose some methods on how to stabilize training for GANs such as pretraining method. In this paper, we adopt their pretraining method before normal training process.  

It should be noted that, although we use images as one source of inputs, our task is different from image captions \cite{dai2017towards} and VQA tasks \cite{wu2017you}, where images are most important part. In our task, we design multi-modal generator to generate short product titles and mainly consider information from long product titles, with additional information from product image and attribute tags.

\section{Conclusion}

In this paper, we propose a multi-modal generative adversarial network for short product title generation in E-commerce. Different from previous methods which mainly consider information from long product titles, we design a multi-modal generative model to consider additional information from product image and attribute tags. Besides, we focus on overall quality of the generated short titles and evaluate them in a human-like view.
% Experimental results verify the effectiveness of the proposed method on a large E-commerce dataset and the online deployment in a real environment of an E-commerce app. 
Experimental results verify the effectiveness of the proposed method on a large E-commerce dataset, and the online deployment in a real environment of an E-commerce app shows that our method improves the click through rate by 1.66\% and click conversion rate by 1.87\%, respectively.
